Probing to Minimize

We develop approximation algorithms for set-selection problems with deterministic constraints, but random objective values, i.e., stochastic probing problems. When the goal is to maximize the objective, approximation algorithms for probing problems are well-studied. On the other hand, few techniques are known for minimizing the objective, especially in the adaptive setting, where information about the random objective is revealed during the set-selection process and allowed to influence it. For minimization problems in particular, incorporating adaptivity can have a considerable effect on performance. In this work, we seek approximation algorithms that compare well to the optimal adaptive policy. We develop new techniques for adaptive minimization, applying them to a few problems of interest. The core technique we develop here is an approximate reduction from an adaptive expectation minimization problem to a set of adaptive probability minimization problems which we call threshold problems. By providing near-optimal solutions to these threshold problems, we obtain bicriteria adaptive policies. We apply this method to obtain an adaptive approximation algorithm for the MIN-ELEMENT problem, where the goal is to adaptively pick random variables to minimize the expected minimum value seen among them, subject to a knapsack constraint. This partially resolves an open problem raised in Goel et. al's "How to probe for an extreme value". We further consider three extensions on the MIN-ELEMENT problem, where our objective is the sum of the smallest k element-weights, or the weight of the min-weight basis of a given matroid, or where the constraint is not given by a knapsack but by a matroid constraint. For all three variations we explore, we develop adaptive approximation algorithms for their corresponding threshold problems, and prove their near-optimality via coupling arguments.

==> itcs-sections/itcs-introduction.tex <==
\newcommand{\leb}[1]{{\leq \frac{B}{#1}}}
\newcommand{\gbk}{{> \frac{B}{k}}}
\newcommand{\gbi}{> \frac{B}{i}}
\newcommand{\lebi}{\leb{i}}
\newcommand{\bucket}{\textsc{bucket}}
\newcommand{\ceiling}[1]{\lceil #1 \rceil}
\newcommand{\minknapsack}{\textrm{$\minelement$-$\knapsack$}}
\newcommand{\metamin}{\alg}


We consider the following stochastic minimization problem archetype. We are given four objects:
\begin{enumerate}
    \item a {ground set} (\emph{universe}) $\universe$ of elements;
    \item a collection of independent non-negative random variables $\{X_e: e \in \universe\}$, which we call \emph{weights} and whose probability distribution is known in advance;
    \item a non-increasing objective function $f(\cdot)$ that maps a set $S \subseteq \universe$ to a non-negative real number based on the realized values of the weights $\{X_e\colon e\in S\}$;
    \item and a constraint, represented as a subset-closed family of feasible sets $\F$.
\end{enumerate}
Our goal is to choose a \emph{selection set} $S \subseteq \universe$ that minimizes $\ex{f(S)}$, subject to the constraint that $S \in \F$.

At a high level, this framework applies to stochastic minimization problems which involve \emph{constrained exploration}. For example, content delivery systems must poll servers to determine content-readiness, and make service decisions in a way that minimizes quality-of-service disruption; a homeowner might request price quotes from contractors and seek to minimize the final cosT paid; venture capital firms must decide which business ventures receive seed funding, and avoid missed growth opportunities.
In the these settings, there is a natural tradeoff between quality assurance and constraint impact which makes these problems hard: often, riskier prospects are ``cheaper’’ but could pay off handsomely, while more stable prospects are either more expensive or have a smaller possible upside.

That said, while many natural stochastic minimization problems exist, most research on stochastic problems has focused on the maximization setting, and there are very few algorithms and techniques capable of handling minimization.
Moreover, while any minimization problem \emph{can} be cast as a maximization problem, the metrics we use to define success are often explicitly skewed one way or another \textemdash especially when optimal results are computationally hard, and we seek approximations. 
For example, consider a test-taking setting where the optimal expected score is a $99$ out of 100. When cast as a maximization problem, any algorithm which obtains an expected score of $50$ is a $2$-approximation, while, when cast as a minimization problem, a $2$-approximation must obtain an expected score of $98$.
In this light, it seems natural that many techniques for approximate maximization do not easily generalize to approximate minimization, and that, in some cases, approximating minimization problems would be incredibly difficult.

One example of a successfully studied stochastic minimization problem is the $\minelement$ problem of \citet{HowToProbe}, a direct inspiration for this work.
As the name suggests, in the $\minelement$ problem, the objective is to choose a set $S$ which minimizes $\ex{\min_{e \in S}{X_e}}$, where the selection set $S$ must satisfy a knapsack constraint.
In particular, \citeauthor{HowToProbe} considered the \emph{non-adaptive} version of this problem, wherein one commits to a set $S$ before learning any of the weights $\{X_e : e \in S \}$.
This is in contrast to the \emph{adaptive} version of this problem, where a policy $\pi$’s selection set $\spi$ is built element-by-element, and an element’s weight is revealed immediately after it is added to the selection set, allowing an adaptive policy to \emph{adapt} its element selections based on the weight outcomes seen so far.
For the non-adaptive version of the $\minelement$ problem, they gave a non-adaptive bicriteria approximation to the best possible non-adaptive policy, and left open the question of approximating the optimal adaptive policy.


The aim of approximating the optimal adaptive policy is an important one. In many settings \textemdash and for minimization problems in particular \textemdash making use of adaptivity can have a profound effect on the objective value. Although for many maximization problems, the gap between the performance of adaptive and non-adaptive algorithms, the so-called \emph{adaptivity gap}, is relatively small, this is not the case for even some very basic minimization problems.
In fact, one can construct simple examples for which the adaptivity gap is arbitrarily large; see Example~\ref{ex:adapgap} in Appendix~\ref{sec:appendix} for an example where there are only $3$ elements to choose from.
As such, for minimization problems especially, we would like to find adaptive solutions which provably compare well to the optimal \emph{adaptive} policy. We do exactly this, for a few select problems.



\subsection{Our results}
For the $\minelement$ problem, \citet{HowToProbe} showed that approximating the optimal non-adaptive policy without augmenting the allowed budget is NP-hard. Given the apparent further complexity of the adaptive setting, we too focus on providing efficiently computable bicriteria approximations to the problems we treat. In particular, we call an algorithm $\pi$ an $(\alpha, \beta)$ approximation if the selection set $\spi$ is the union of at most $\beta$ feasible sets, and $\ex{f\left(\spi\right)}$ is at most $\alpha$ times larger than the optimal expected objective value. 

We give a brief overview of our approximation results. Our initial result is an adaptive approximation for the $\minknapsack$ problem, an adaptive version of the $\minelement$ problem treated in \cite{HowToProbe}. Afterwards, we present further results on three variations on the $\minknapsack$ problem, which we describe there.
% First, we discuss a strict generalization of the $\minknapsack$ problem, where the knapsack constraint is maintained, and the objective function is now the sum of the $k$ smallest elements probed; we call this the $\mink$-$\knapsack$ problem. Then, we alter this new problem to have a matroid constraint instead of a knapsack constraint, developing approximation results for the $\mink$-$\matroid$ problem. Finally, in the $\minbasis$-$\cardinality$ problem, we generalize the objective function to be the weight of the minimum weight basis contained in the selection set, given some matroid, and simplify the constraint to a simple cardinality constraint.

\subsubsection{\textbf{$\minknapsack$ problem}} In Section~\ref{sec:min-ele}, we treat the $\minelement$ problem specifically in the setting where weights take values in $\intdomain \triangleq \{0,1,2,\dots, m \}$, resolving an open question of \cite{HowToProbe} about techniques for approximating the adaptive version of the $\minelement$ problem.

\begin{restatable}{theorem}{RESTATEthmminele}
\label{thm:min-ele}
For the $\minone$-$\knapsack$ problem where the random variables take values in $\intdomain$, there exists an adaptive policy that obtains a $\mineleapprox$-approximation.
\end{restatable}

\subsubsection{\textbf{$\mink$-$\knapsack$ problem}}\label{sec:mink-knap-intro}
In Section~\ref{sec:mink-knap}, we investigate an extension to the $\minknapsack$ problem that we refer to as the $\mink$-$\knapsack$ problem. In the $\mink$-$\knapsack$ problem, we maintain the previous knapsack constraint, but now make our objective function $f(S)$ to be the sum of the smallest $k$ weights in $S$.

\begin{restatable}{theorem}{RESTATEthmminkknap}\label{thm:mink-knap}
    For the $\mink$-$\knapsack$ problem where the random variables takes values in $\intdomain$, there exists an adaptive policy that obtains a $\minkknapapprox$-approximation.
\end{restatable}


\subsubsection{\textbf{$\mink$-$\matroid$ problem}}
In Section~\ref{sec:mink-mat}, we investigate the $\mink$-$\matroid$ problem, where the objective function $f(S)$ is again the sum of the smallest $k$ weights in the selection set $S$, but the constraint is a matroid constraint.
More explicitly, we are given a matroid $\Mouter = (\universe, \I)$ that we refer to as the outer matroid, specified by the ground set $\universe$ and a family of independent sets $\I$. Our constraint is that a selection set $\spi$ is feasible if and only if it is an independent set, i.e., $S$ lies in the family of feasible sets $\F = \I$.
\begin{restatable}{theorem}{RESTATEthmminkmat}\label{thm:mink-mat}
    For the $\mink$-$\matroid$ problem where the random variables take values in $\intdomain$, there exists an adaptive policy that obtains a $\minkmatapprox$-approximation.
\end{restatable}


\subsubsection{\textbf{$\minbasis$-$\card$ problem}}
In Section~\ref{sec:minbasis-card}, we investigate the $\minbasis$-$\card$ problem, where the objective function $f$ \emph{generalizes} the $\mink$ objective to a function specified by a matroid $\Minner=(\universe,\I)$ that we refer to as the inner matroid.
Specifically, for the $\mink$ objective, one can consider the the smallest $k$ elements in $\spi$ as the minimum weight basis for the matroid where the independent sets are sets consisting of at most $k$ elements; this matroid is typically called the uniform matroid of rank $k$. 
For the $\minbasis$ objective, we generalize the uniform matroid to a general matroid $\Minner$, allowing the objective function $f(S)$ to become the weight of the minimum-weight basis of $\Minner$ contained in $S$.
To account for this increased complexity, we simplify the constraint to a simple cardinality constraint, i.e., we require that $\abs{\spi} \leq B$.

\begin{restatable}{theorem}{RESTATEthmminbasiscard}\label{thm:minbasis-card}
    For the $\minbasis$-$\cardinality$ problem where the random variables takes values in $\intdomain$, there exists an adaptive policy that obtains a $\minbasiscardapprox$-approximation.
\end{restatable}


\subsection{Techniques}

We now describe the main techniques which allow us to prove our results.

\subsubsection{Lemma~\ref{lem:reduction} (Reduction to threshold problems)}
The primary technique we develop and make use of is the reduction of Lemma~\ref{lem:reduction}, which is built on the notion of a threshold problem. The $f$-$\F$  threshold problem with threshold $t$  is an adaptive probability minimization problem, wherein the policy $\pi$ tries to avoid $f(\spi) > t$ with as high a probability as possible. Lemma~\ref{lem:reduction} says that, given an $(\alpha, \beta)$-approximation for the $f$-$\F$ threshold problem, one can construct a $\left(4\alpha, O(\log\log{m})\beta  \right)$-approximation for the adaptive expectation minimization problem $\min_{\pi \in \adm{\F}}{\ex{f(\spi)}}$.

\begin{restatable*}[\textbf{Reduction to threshold problems}]{lemma}{RESTATElemreduction}\label{lem:reduction}
Let $f(S)$ be a non-increasing objective function taking values in $\intdomain$ for a positive integer $m$. Let $\F$ be the constraint family and $\adm{\F}$ be the set of feasible policies under $\F$.  Suppose that for any $t \in \intdomain$, the $f$-$\F$ threshold problem
\begin{equation*}
    \min_{\pi \in \adm{\F}}{\pr{f\left(\spi\right) > t }}
\end{equation*}
admits an $(\alpha,\beta)$-approximation.  Then the stochastic minimization problem 
\begin{equation*}
\min_{\pi \in \adm{\F}}{\ex{f\left(\spi\right)}}
\end{equation*}
admits a $(4\alpha, O(\log\log m)\cdot \beta)$-approximation.
\end{restatable*}

We prove Lemma~\ref{lem:reduction} by constructing a meta-algorithm which can make calls to the threshold problem approximation $\threshapprox$. The main idea at work here is to build around decompositions of $\ex{f(\spi)}$. First, observe the decomposition of $\ex{f(\spi)}$ as a sum of probabilities $\pr{f(\spi) > t}$. Intuitively, a good policy for our problem should somehow simultaneously minimize all of these $\pr{f(\spi)>t}$ terms. Moreover, because we are explicitly seeking approximations, one need not actually minimize all of these terms. Since 
\begin{equation*}
\ex{f\left(\spi\right)}\le\pr{f\left(\spi\right)>0}+\sum_{j=0}^{\lfloor \log m\rfloor}\pr{f\left(\spi\right)>2^j}2^j \le 2\ex{f\left(\spi\right)}.
\end{equation*}
we can restrict our focus to thresholds which are powers of 2.

If one uses $\threshapprox$ to $(\alpha, \beta)$-approximate the $f$-$\F$ threshold problem for every threshold that’s a power of $2$, then one obtains a $\left(2\alpha, O(\log{m})\beta\right)$-approximation to the optimal adaptive policy. 
However, the adaptivity of our setting makes calling $\threshapprox$ on a fixed set of thresholds incredibly wasteful. Since $f(\cdot)$ is non-increasing, once we have obtained $f(\spi) \leq t$, we need not worry about solving threshold problems with thresholds larger than $t$. 
To make use of this monotonicity, we instead perform adaptive binary search to determine the next threshold to call $\threshapprox$ on. 
To handle an edge case, we first call $\threshapprox$ on the threshold $0$, adaptively probing the set $S_0$. 
If we obtain $f(S_0) = 0$, then clearly we can stop and return $S_0$. 
Otherwise, we perform the following procedure: Starting with the median threshold $t$, if the $\threshapprox$ probes a set $S_t$ and succeeds in obtaining $f(S_t) \leq t$, then we recurse on the thresholds smaller than $t$; if $\threshapprox$ fails to obtain $f(S_t) \leq t$, then we recurse on the set of thresholds larger than $t$. 
One should note the asymmetry between success and failure here: success at a threshold $t$ guarantees $\metamin \leq t$ from then on, but failure at $t$ \emph{does not} guarantee that $\metamin > t$ from then on. 
Nevertheless, one can construct an upper bound $\ub$ on $\metamin$ by analyzing $\metamin$ as if failure at $t$ \emph{does} imply $\metamin > t$ from then on. 
From the basic stopping conditions, it follows easily that, for adjacent thresholds $a$ and  $b$ in our powers-of-2 set,
\begin{equation*}
\pr{\ub \in (a, b]} = \pr{\text{$\metamin$ fails at $a$ and succeeds at $b$}} \leq \pr{f(S_a) > t}.
\end{equation*}
When combined with the powers-of-2 decomposition mentioned earlier, this is enough to show the lemma.




\subsubsection{Corollary~\ref{coro:sum-of-k} (Sum-of-$k$ reduction)}
In Corollary~\ref{coro:sum-of-k}, we extend the reduction of Lemma~\ref{lem:reduction} to work with objective functions of the form $f(S) = \sum_{i=1}^k{g_i(S)}$, where the $g_i(\cdot)$ is monotonic in $i$.  Our main idea here is again based on a decomposition of $\ex{f(\spi)}$. In particular, we notice that, if $f(S) = \sum_{i=1}^k{g_i(S)}$ where the $g_i(\cdot)$ are non-increasing in $i$,
\begin{equation*}
    \ex{\sum_{i=1}^{k}{g_i\left(\spi\right)}}  \leq \ex{ \sum_{j=0}^{\floor{\log(k)}}{g_{2^j}\left(\spi\right)2^j}}\le 2\ex{\sum_{i=1}^{k}{g_i\left(\spi\right)}}.
\end{equation*}
If every function $g_i$ satisfies the preconditions of Lemma~\ref{reduction}, then, at the cost of an additional factor of $2$ in the expected value and factor of $\log{k}$ in resource augmentation, we can simply use our meta-algorithm $\metamin$ to directly optimize for $\ex{g_i(\spi)}$ on specifically the indices $i$ which are powers of $2$. Doing this gives us Corollary~\ref{coro:sum-of-k}.
 
 \begin{restatable*}[\textbf{Sum-of-$k$ reduction}]{coro}{RESTATEcorosumofk}
\label{coro:sum-of-k}
    Let $g_i(S)$, $i \in [k]$, be a non-increasing function taking values in $\intdomain$, and assume that the function sequence $(g_i)$ is monotonic in $i$.  Let $f(S) = \sum_{i=1}^k{g_i(S)}$. Suppose that for any $t \in \intdomain$, the $g_i$-$\F$ threshold problem 
    \begin{equation*}
    \min_{\pi \in \adm{\F}}{\pr{g_i\left(\spi\right) > t }}
    \end{equation*}
    admits an $(\alpha, \beta)$-approximation. Then the stochastic minimization problem 
    \begin{equation*}
    \min_{\pi \in \adm{\F}}{\ex{f\left(\spi\right)}}
    \end{equation*}
    admits an $(8\alpha,  O(\log\log m\cdot \log k) \cdot \beta)$ approximation.
\end{restatable*}
 
\subsubsection{The $\minknapsack$ problem}
Armed with the reduction in Lemma~\ref{lem:reduction}, the proof of Theorem~\ref{thm:minelement} is complete as soon as we obtain a $(1,2)$-approximation to the $\minknapsack$ threshold problem
\begin{equation*}
    \min_{\pi \in \adm{\F}}{\pr{\min_{e \in \spi}{X_e} > t}}.
\end{equation*}
We discuss the analysis of our threshold algorithm before describing it. Note that any policy $\pi$ succeeds at obtaining $\min_{e\in S}{X_e} \leq t$ as soon as it finds a single element for which $X_e \leq t$. It follows that adaptivity adds nothing to solving this problem, so that we might as well concern ourselves with the non-adaptive problem
\begin{equation*}
    \min_{S \in \F}{\pr{\min_{e\in S}{X_e} > t}}.
\end{equation*}
Taking the logarithm of the objective, there’s a straightforward reduction from this problem to a knapsack instance where each element has \emph{reward}  $-\log{\pr{X_e > t}}$.
It follows easily that the following procedure gives a set with at least optimal knapsack value: 
\begin{itemize}
    \item Start with an empty set $S$. 
    \item While the $\cost{S} < B$, add to $S$ the unprobed element with the largest \emph{reward density} $\frac{\reward{e}}{c_e}$.
\end{itemize}
Furthermore, the final element costs at most $B$, giving us the $\mineleapprox$-approximation which completes Theorem~\ref{thm:min-ele}.

\subsubsection{The $\mink$-$\knapsack$ problem}
We turn next to a strict extension of the $\minknapsack$ problem: the $\mink$-$\knapsack$ problem. The first step, like in the $\minknapsack$ problem, is to apply a threshold-based reduction. This time, though, we make use of Corollary~\ref{coro:sum-of-k}. Observe that, if $y_i(S)$ is the weight of the $i$-th smallest weight element in $S$, then our objective $f(S)$,  the sum of the $k$ smallest weights in $S$, is simply $\sum_{i=1}^k{y_i(S)}$. Applying the threshold-based reduction of Corollary~\ref{coro:sum-of-k}, we need only find a $(1, O(\log{k})$-approximation to the threshold problem
\begin{equation*}
    \min_{\pi \in \adm{\F}}{\pr{y_i(\spi) > t}}.
\end{equation*}
The threshold problem here is interesting in its own right, and can be conceptualized in the following way:
\begin{problem*}[\textbf{The $i$-heads problem}]
Say we have a set of coins $\universe$ to choose from, each having its own cost $c_e$ and heads-probability $p_e$. Upon purchasing a coin, we flip it once. Given a budget $B$, the $i$-heads problem is to adaptively purchase coins in a way that maximizes $\pr{\text{at least $i$ coins land heads}}$.
\end{problem*}
The mapping between these problems is simple: an element $e$ which has a below-threshold weight is equivalent to a coin $e$ which comes up heads. For ease of exposition, we describe our $(1,O(\log{k}))$-approximation in terms of the $i$-heads problem.

When the number of heads needed $i$ is simply $1$, our treatment of the $\minknapsack$ problem tells us that the following overflowing-greedy algorithm has an at-least-optimal probability of success:
\begin{itemize}
    \item Begin with an empty set $S$.
    \item While $\cost{S} < B$, add to $S$ the unprobed element  $e$ with the largest \emph{reward density} $\frac{\reward{e}}{c_e} = \frac{- \log{ (1- p_e)}}{c_e}$.
\end{itemize}
We extend this strategy to the general $i$ via the algorithm $\greedyalg(\universe, B, i, t)$. It operates in precisely the same way as $\minknapsack$’s overflowing-greedy algorithm, but \emph{extends} the available budget from $B$ to $B + k\delta$, where $\delta$ is the maximum cost of any element in $\universe$.

The proof that $G= \greedyalg(\universe, B, i, t)$ outperforms any admissible policy $\pi$ is particularly interesting; there are four steps. In the first step, we decompose $\pi$’s decision tree based on when it obtains its first head, and, using this decomposition, derive an implicit expression for a policy’s success probability.

In the second step, we use this expression to make a visual argument for a sufficient condition which would imply
\begin{equation*}
    \pr{\text{$G$ obtains $\geq i$ heads}} \geq \pr{\text{$\pi$ obtains $\geq i$ heads}}.
\end{equation*}
The main idea of this step is to approach the success probability of $\pi$ as the discrete integral of a non-increasing function, i.e., the total area covered by a series of rectangles of declining height and growing width. From this observation, to show that $G$ succeeds more often than $\pi$, it suffices to show that the integrand for $G$ dominates the integrand for $\pi$, or, equivalently, that every rectangle of $\pi$ is completely covered by at least one rectangle of $G$; see Figure~\ref{fig:rect-decomp-tikz} for a visualization.

% The general idea is to construct a sequence of rectangles, where the width of the $j$-th rectangle is the probability that $\pi$ has obtained a head by the $j$-th element probed, and the height of the $j$-th rectangle is the probability that $\pi$ obtains $i$ heads, given that $\pi$ has obtained a head \emph{on} the $j$-th element probed. From the law of the total probability, it follows that the success probability of $\pi$ is simply the total area covered by these rectangles, and to show that $G$ is better than $\pi$, it suffices to show that every rectangle of $\pi$ is completely covered by at least one rectangle of $G$.


In the third step, we begin proving that this “rectangle covering” condition holds via induction on the heads-target $i$. Our initial move is to modify $\pi$ into a surrogate policy $\pitilde$ which is easier to analyze. We make $\pitilde$ run $\pi$ until obtaining its first heads, and afterwards switch to $\greedyalg$ with the remaining budget. By our inductive assumption, the rectangles of $\pitilde$ can only be made larger by doing this, so it suffices to show our covering condition for $G$ and $\pitilde$ instead.

In the fourth and final step, we prove that $G$ covers $\pitilde$ via a neat coupling argument. We make use of the following important observation: because $G$ is a deterministic set, the order in which we flip the coins of $G$ has no bearing on the number of coins that land heads. The gist of the argument is to show that there exists an ordering of $G$ such that
\begin{itemize}
    \item The policies $G$ and $\pitilde$ probe the same set after obtaining their first heads.
    \item For any amount of remaining budget $B’$, the probability that $G$ obtains its first heads with $B’$ budget remaining is greater than the probability that $\pi$ obtains its first heads with $B’$ budget remaining.
\end{itemize}
In the end, this argument shows that $G$ stochastically dominates every policy $\pi \in \adm{\F}$, in that, for all $\ell \in [i]$, 
\begin{equation*}
    \pr{\text{$G$ obtains $\geq \ell$ heads}} \geq \pr{\text{$\pi$ obtains $\geq \ell$ heads}}.
\end{equation*}
Combined with the fact that $\cost{G} \leq B + (k+1)\delta$, we have a promising algorithm for the $i$-heads problem.

Unfortunately, without additional intervention, the max cost of a coin could be $~B$, which would make the $B + (k+1)\delta$ cost of this extended greedy approach prohibitively expensive. To counteract this, we use the binning procedure $\bin(\universe, B, i, t)$ to construct a set $\binset$ such that, when used with the low-cost greedy set $G’ = \greedyalg\left(\{ e \in \universe : c_e \leq B\}, B, i, t \right)$, the combined set $\binset \cup G’$ has a higher success probability than any admissible policy $\pi$.

We achieve this by defining $\bucket_j$ as $\left \{e \in \universe : \frac{B}{2^{j-1}} \geq c_e > \frac{B}{2^{j}} \right\}$, making $C_j$ the $2^j$ elements in $\bucket_j$ with the highest heads-probabilities, then taking $\binset = \cup_{j=1}^{\ceiling{\log{i}}}{C_j}$. 
In a direct coupling sense, the elements of $\binset$ are ``better'' than the high-cost elements of any non-augmented selection set. This, it turns out, is enough to show the theorem.

\subsubsection{The $\mink$-$\matroid$ problem}
We now discuss our treatment of our first matroid-based variation on the $\mink$-$\knapsack$ problem, the $\mink$-$\matroid$ problem. By virtue of Corollary~\ref{coro:sum-of-k}, proving Theorem~\ref{thm:mink-mat} again reduces to providing a $(1, O(1))$-approximation of the $y_i$-$\matroid$ threshold problem, where recall that $y_i(S)$ is the $i$-th smallest weight in $S$.
= We show that the typical matroid greedy algorithm $\matgreedy$, described in Algorithm~\ref{alg:mink-mat}, is an optimal policy for this problem. In fact, the matroid greedy algorithm stochastically dominates any other policy. We argue this via induction on the matroid rank of the constraint. The main observation one must make here is that, after probing a single element, we find ourselves in a problem state which is nearly exactly like the starting state, but with a possibly reduced number of heads, and a resulting constraint family which is a matroid with a strictly smaller rank.

\subsubsection{The $\minbasis$-$\cardinality$ problem}
We now discuss the treatment of our final problem, the $\minbasis$-$\cardinality$ problem. The proof of Theorem~\ref{thm:minbasis-card} is again through Corollary~\ref{coro:sum-of-k}.
However, it is not obvious how we can write our objective $f(S)$ as $\sum_{i=1}^k{g_i(S)}$ for a monotonic function sequence $(g_i(\cdot))$ where each $g_i(\cdot)$ is a non-decreasing function taking values in $\intdomain$.
In our proof, we first show that we can specify $g_i(S)$ to be the $i$-th smallest element in the minimum-weight basis contained in $S$ generated by the matroid greedy algorithm.
Then we show inductively that $\adapgreedy$, a simple adaptive matroid greedy algorithm described in Algorithm~\ref{alg:minbasis-card}, is optimal for the resulting $g_i$-$\cardinality$ threshold problem.
The key idea here is, again, to use our inductive assumption to reason about the future behavior of an optimal policy.

